Problematic Tokens: Tokenizer Bias in Large Language Models

Recent advancements in large language models(LLMs), such as GPT-4 and GPT-4o, have shown exceptional performance, especially in languages with abundant resources like English, thanks to extensive datasets that ensure robust training. Conversely, these models exhibit limitations when processing under-resourced languages such as Chinese and Korean, where issues including hallucinatory responses remain prevalent. This paper traces the roots of these disparities to the tokenization process inherent to these models. Specifically, it explores how the tokenizers vocabulary, often used to speed up the tokenization process and reduce tokens but constructed independently of the actual model training data, inadequately represents non-English languages. This misrepresentation results in the propagation of under-trained or untrained tokens, which perpetuate biases and pose serious concerns related to data security and ethical standards. We aim to dissect the tokenization mechanics of GPT-4o, illustrating how its simplified token-handling methods amplify these risks and offer strategic solutions to mitigate associated security and ethical issues. Through this study, we emphasize the critical need to rethink tokenization frameworks to foster more equitable and secure AI technologies. The code and data are available at https://github.com/yeyimilk/LLMGPT4o

==> sec/1_introduction.tex <==
\section{Introduction}


% The advent of Large Language Models (LLMs) such as GPT-4 and BERT has revolutionized various applications in natural language processing (NLP). These models rely on vast corpora for training, which ideally should be representative and free from noise. However, corpus pollution, where infrequent or abnormal tokens are overrepresented, can undermine the reliability of LLMs. This paper investigates the extent of corpus pollution and its impact on LLM outputs, with a focus on security implications.

% In the burgeoning field of artificial intelligence, the efficacy and fairness of large language models (LLMs) such as OpenAI's GPT series are heavily contingent upon the diversity and quality of their training data \cite{brown2020language}. The foundational premise that more data equates to better performance underpins the current approaches to LLM development \cite{yan2023autocast, chang2024survey}. However, this premise is significantly challenged by issues of access and data quality, especially in non-English languages such as Chinese. Unlike in more open environments where vast swathes of text data are freely accessible, in China, stringent data control measures and privacy laws tightly regulate the collection and use of digital content.

% Most of the high-quality, contextually rich data in Chinese remains locked within app servers and proprietary databases, protected by rigorous anti-scraping measures, including sophisticated CAPTCHAs and legal constraints. This situation necessitates reliance on publicly available data sources, which, unfortunately, are often riddled with low-quality content such as gambling and pornography links or are skewed by excessive promotional material. The implications of training LLMs on such datasets are profound, affecting not only the model's linguistic capabilities but also its ethical alignment, as evidenced by biases and hallucinations in the generated text.

% Furthermore, the reliance on low-quality open-access websites as primary data sources raises significant ethical concerns. These concerns include privacy infringements, potential breaches of copyright, and the perpetuation of misinformation. This paper aims to explore these challenges specifically within the context of Chinese language data, assessing the impact of limited and biased datasets on LLM performance. We also propose mitigation strategies aimed at improving data acquisition practices and enhancing model robustness and ethical compliance. By addressing these issues, we contribute to the broader discourse on the responsible development of AI technologies, ensuring they are both effective and equitable across diverse linguistic landscapes.
In the burgeoning field of artificial intelligence, the efficacy and fairness of large language models (LLMs) such as OpenAI’s GPT series are heavily contingent upon the diversity and quality of their training data\cite{brown2020language}. The foundational premise that more data equates to better performance underpins current approaches to LLM development\cite{yan2023autocast, chang2024survey}. However, this premise is significantly challenged by access and data quality issues, particularly in non-English languages like Chinese and Korean. These languages not only demonstrate reduced performance but also amplify security and ethical issues due to the limited and often biased data available for model training.

% Most of the high-quality, contextually rich data in Chinese remains locked within app servers and proprietary databases, protected by rigorous anti-scraping measures, including sophisticated CAPTCHAs and legal constraints. This situation necessitates reliance on publicly available data sources, which, unfortunately, are often riddled with low-quality content such as gambling and pornography links or are skewed by excessive promotional material. Training LLMs on such datasets can profoundly impact the model’s linguistic capabilities and ethical alignment, leading to biases and hallucinations in the generated text.
Unlike more open environments where vast swathes of text data are freely accessible, regions like China enforce stringent data control measures and privacy laws that tightly regulate the collection and use of digital content. Most of the high-quality, contextually rich data in Chinese remains locked within app servers and proprietary databases, protected by rigorous anti-scraping measures, including sophisticated CAPTCHAs and legal constraints. This situation necessitates reliance on publicly available data sources, which, unfortunately, are often riddled with low-quality content such as gambling and pornography links or are skewed by excessive promotional material. Training LLMs on such datasets can profoundly impact the model’s linguistic capabilities and ethical alignment, leading to biases and hallucinations in the generated text.


To illustrate these data challenges, Fig \ref{fig: token_samples} presents the abnormal tokens identified in Chinese text. These tokens were translated into English and manually classified, revealing that most long tokens involve gambling and adult content. Our analysis revealed that most of the long tokens involve gambling and adult content. This underscores the ethical implications of relying on publicly available data sources that may contain such inappropriate content.


The reliance on low-quality open-access websites as primary data sources also raises significant ethical concerns, including privacy infringements, potential breaches of copyright, and the perpetuation of misinformation. This paper aims to explore these challenges specifically within the context of Chinese language data, assessing the impact of limited and biased datasets on LLM performance. We also propose mitigation strategies aimed at improving data acquisition practices and enhancing model robustness and ethical compliance. By addressing these issues, we contribute to the broader discourse on the responsible development of AI technologies, ensuring they are both effective and equitable across diverse linguistic landscapes.



\input{sec/table_sample}


\section{Introduction}
% Recent advanced LLMs have shown their great abilities in dealing with different NLP tasks, such as a, b. However, the quality of the LLMs-generated context in some specific domains is still underdeveloped, which requires research and improvement.

% The most recently OpenAI launched model, GPT-4o, has demonstrated its great abilities in understanding audio, vision, and text, as well as its "real-time" responding speed.
% However, it has been shown that GPT-4o generated unrelated output, also known as Hallucination, when dealing with some Chinese content.

% Previous studies about hallucination or generating risky content focused on three key aspects: data, training, and inference. However, only a few talk about the matter of tokenization. 

% It's a fact that the public token library used by GPT-4o, \textit{tiktoken}, has been polluted full of porn and gambling words.

% Our study will show a comprehensive investigation of the performance of GPT-4 and GPT-4o in dealing with these special tokens and how GPT-4o can overcome the hallucination or generate risky content issues(but split the long Chinese sequence input into short texts to avoid the long chinese's correspoding token is appears in the tokenized id vector).


% Recent advancements in large language models (LLMs) have demonstrated remarkable performance across various natural language processing (NLP) tasks, such as text generation and machine translation. Despite these strides, the quality and reliability of LLM-generated content in specific cases remain constrained, warranting further exploration and improvement.

% OpenAI's most recent model, GPT-4o, stands out for its impressive capabilities in understanding and processing audio, vision, and text, coupled with its swift ``real-time" response speed. Nonetheless, GPT-4o exhibits a notable limitation when handling certain Chinese language inputs: it produces content that is nonsensical to the context, a phenomenon also referred to as `hallucination.' This issue compromises the reliability and safety of the outputs, often leading to responses that include gambling or adult material.

% Existing literature exploring the issue of hallucination or the generation of inappropriate content primarily centers around three critical aspects: the preparation and selection of data, the training methodology employed, and the aspects governing inference. In contrast, there is a dearth of studies focusing on the substantial influence of tokenization on model behavior and output.

% A notable concern is the public token library used by GPT-4o, known as \textit{tiktoken}, which contains a significant number of tokens associated with pornography and gambling. This contamination within the token library exacerbates the issue, leading to undesirable outputs when the model encounters specific Chinese inputs.

% In this study, we conduct a comprehensive investigation into the performance differences between GPT-4 and GPT-4o when processing these special tokens. We demonstrate how segmenting those special long Chinese sequences into shorter texts can mitigate the hallucination and risky content generation issues in GPT-4o by preventing the problematic tokens from appearing in the tokenized input vector. Through our findings, we aim to provide actionable insights for enhancing the robustness and safety of future LLM deployments.

==> sec/2_Relatedwork.tex <==
\section{Related Work}

% The training of large language models (LLMs) is critically influenced by the quality and diversity of their training datasets. Issues such as dataset bias and data quality have been well-documented in the literature, highlighting the challenges in developing ethically aligned and universally applicable AI systems. For instance, the landmark paper by Gebru et al. (2021)\cite{gebru2021datasheets} on "Datasheets for Datasets" emphasizes the importance of transparency in dataset creation processes to mitigate biases inherent in machine learning models.

% Corpus pollution—where training data are contaminated with misleading or inappropriate content—has significant implications for model output. Bender and Friedman (2018)\cite{bender2018data} explored the consequences of such pollution in their critical work, warning of the dangers of over-relying on automated processes without sufficient oversight, particularly in sensitive applications.

% In terms of linguistic diversity, challenges specific to non-English languages are often underrepresented in mainstream AI research. Koehn and Knowles (2017)\cite{koehn2017six} highlighted the scarcity of resources and research for many languages, which limits the development of effective NLP tools outside of widely spoken languages. This scarcity is particularly problematic given the increasing global use of LLMs.

% With regard to mitigation strategies, recent research has proposed various techniques to improve the quality of training data. Raffel et al. (2020)\cite{roberts2019exploring} in their exploration of the T5 model discuss methods to curate and filter data to enhance model reliability and fairness. They demonstrate how careful consideration of data sources and preprocessing steps can significantly impact model outputs.

% This paper contributes to these discussions by focusing on the specific challenges of acquiring and utilizing high-quality training data for LLMs in non-English contexts. We address the localized constraints on data collection, exacerbated by strict data governance, and the prevalence of low-quality public data sources. By integrating novel mitigation strategies and showcasing their effectiveness, our work seeks to enhance the ethical alignment and functionality of LLMs across diverse linguistic landscapes, providing valuable insights that can be applied to other languages facing similar issues.

The quality and diversity of training datasets significantly influence the training of LLMs, with well-documented impacts on both model performance and ethical alignment. Recent controversies, such as biases in language generation and ethical misalignments in AI applications, underscore the urgency of addressing these issues. Studies like Gebru et al. (2021) have introduced "Datasheets for Datasets," emphasizing transparency in dataset creation to mitigate inherent biases.Their work underscores the need for clear documentation and ethical considerations in data handling \cite{gebru2021datasheets}.

% The training of LLMs is critically influenced by the quality and diversity of their training datasets. Issues such as dataset bias and data quality have been well-documented in the literature, highlighting the challenges in developing ethically aligned and universally applicable AI systems.

% Gebru et al. introduced the concept of "Datasheets for Datasets," emphasizing the importance of transparency in dataset creation processes to mitigate biases inherent in machine learning models. 

Corpus pollution, where training data are contaminated with misleading or inappropriate content, has significant implications for model output. Bender and Friedman explored the consequences of such pollution, warning of the dangers of over-relying on automated processes without sufficient oversight, particularly in sensitive applications \cite{bender2018data}.

In terms of linguistic diversity, challenges specific to non-English languages are often underrepresented in mainstream AI research. Koehn and Knowles highlighted the scarcity of resources and research for many languages, which limits the development of effective NLP tools outside of widely spoken languages \cite{koehn2017six}. This scarcity is particularly problematic given the increasing global use of LLMs.

Recent research has proposed various techniques to improve the quality of training data. Raffel et al., in their exploration of the T5 model, discussed methods to curate and filter data to enhance model reliability and fairness. They demonstrated how careful consideration of data sources and preprocessing steps can significantly impact model outputs \cite{roberts2019exploring}.

This paper contributes to these discussions by focusing on the specific challenges of acquiring and utilizing high-quality training data for LLMs in non-English contexts. We address the localized constraints on data collection, exacerbated by strict data governance, and the prevalence of low-quality public data sources. By integrating novel mitigation strategies and showcasing their effectiveness, our work seeks to enhance the ethical alignment and functionality of LLMs across diverse linguistic landscapes, providing valuable insights that can be applied to other languages facing similar issues.


==> sec/6_Case_Study.tex <==
\section{Case Study: Ethical Implications of Misleading Token Usage}

\subsection{Background}
The term \BeijingPK{} seems innocuous and can be straightforwardly translated into English as ``Beijing Racing(BR).'' However, it carries significant contextual nuances that vary widely depending on the source. Traditionally, ``Beijing Racing'', refers to a government-supported welfare lottery in China, intended for fund-raising for public welfare activities. This original context suggests a legitimate and ethical activity.

\subsection{Problem Identification}
Despite its official designation in everyday usage, BR frequently alludes to illicit gambling and fraud activities. This divergence between its official and common vernacular usages presents substantial challenges for LLMs trained on web-scraped data, which may not adequately distinguish between these contexts.

\subsection{Methodology}
To investigate how BR is represented in datasets likely used for training LLMs, we analyzed the top 20 search results from Google and Baidu. Our analysis focused on assessing the nature of the content linked with the term and evaluating the implications of this content on the quality of training data.

\subsection{Findings}
Our analysis revealed that 95\% of the web pages associated with BR were primarily gambling sites, often unofficial and illegal. This prevalent misrepresentation in training data can mislead LLMs to associate the term more with illegal activities rather than its legitimate context, highlighting a critical area of ethical concern in data sourcing.

% The analysis indicated that a significant majority of the web pages (38 out of 40) associated with BR  were linked to gambling sites, many of which are unofficial and potentially illegal. This prevalent association suggests that an LLM trained on such data will likely misconstrue BR as primarily related to gambling rather than its legitimate lottery context.

\subsection{Ethical Implications}
The potential misrepresentation of BR  in LLMs outputs poses several ethical issues:
\begin{itemize}
    \item \textbf{Misinformation}: Highlighting the term predominantly in connection with illegal activities could mislead users regarding the legality and nature of BR.
    \item \textbf{Legal Risks}: Content generated that inadvertently promotes or normalizes gambling might lead to legal consequences in regions where gambling is stringently regulated or prohibited.
    \item \textbf{Cultural Sensitivity}: Inaccurate representation of local cultural and legal contexts can result in outputs that are culturally insensitive or inappropriate.
\end{itemize}

\subsection{Mitigation Strategies}
To mitigate these risks, we propose the following strategies:
\begin{enumerate}
    \item \textbf{Enhanced Data Filtering}: Implement advanced filtering algorithms to identify and exclude content from unreliable or illegal sources during the data collection process for training LLMs.
    \item \textbf{Contextual Awareness in Modeling}: Develop models capable of understanding and differentiating between the multiple contexts and meanings of specific terms based on additional data cues.
    \item \textbf{Ethical Review Processes}: Establish rigorous review processes to assess and refine training datasets and model outputs, particularly for terms known to have dual meanings or sensitive implications.
\end{enumerate}


==> sec/BG_backup.tex <==
\subsection{Background}


% Corpus pollution refers to the presence of atypical or erroneous data within the training set of an LLM. Such data can distort the model's understanding and generation of language, leading to unreliable or incorrect outputs. This issue becomes critical in applications requiring high accuracy and trustworthiness, such as medical advice, legal interpretations, and security-sensitive communications.
Corpus pollution, the infiltration of atypical or erroneous data into a language model's training set, poses significant challenges for the development of reliable and effective large language models (LLMs). Such data can skew a model’s language comprehension and output, leading to the generation of inaccurate or misleading information. This issue is crucial in contexts requiring precise and trustworthy communication, such as medical diagnostics, legal advisement, and security protocols.

\textbf{Real-world Example}: In our analysis, we identified problematic tokens in the tokenizers of models like GPT-4o, particularly in Chinese and Korean. Many long tokens from these languages were associated with gambling, sexual content, and phishing. These findings are indicative of the types of corpus pollution that not only compromise the relevance and safety of the generated content but also potentially introduce severe biases. For example, certain long Chinese tokens were predominantly linked to gambling and adult content, while similar issues were observed with Korean tokens related to adult content. Such tokens illustrate how corpus pollution can introduce significant risks and biases into LLM outputs.

Distinct from general data quality and accessibility concerns, corpus pollution specifically addresses the integrity and representativeness of data within the training set. While LLMs are often touted for their ability to improve with larger datasets, the presence of polluted data can paradoxically degrade their performance, especially when such data is not immediately evident due to its embedded nature in large-scale datasets. The risks associated with polluted data are not merely technical but also ethical, as they can perpetuate misinformation and bias, which are especially problematic in sensitive applications.

% Addressing corpus pollution requires an understanding of its sources—ranging from maliciously crafted entries to subtle biases in content collection processes. This background sets the stage for discussing targeted mitigation strategies that go beyond broad data collection improvements, focusing on enhancing data filtration and validation techniques to refine the quality of datasets used for training sophisticated AI models.

==> sec/table_sample.tex <==



% \begin{table*}[h]
% \centering
% \caption{\small{Classification of abnormal Chinese tokens by content type}}
% \renewcommand{\arraystretch}{1.3}
% \begin{tabular}{lccc}
% \toprule

% Token ID & Token & Translation & Category \\

% \midrule
% 181081 & 微信公众号天天中彩票 & WeChat official account win the lottery every day &  Gambling \\
% 185118 & 日本毛片免费视频观看 & Japanese-produced Adult Content Available for Free Watching & Adult Content \\
% 13492 & 北京赛车 & Beijing Racing & Gambling \\
% 53332 & 国产精品 & Chinese-produced Adult Content & Adult Content \\


% \bottomrule
% \end{tabular}
% \label{tab: token_samples}
% \end{table*}


\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{figs/token_samples.jpg}
    \caption{Classification of abnormal Chinese tokens by content type.}
    \label{fig: token_samples}
\end{figure*}
